Inaudible Adversarial Perturbation: Manipulating the Recognition of User Speech in Real Time

Automatic speech recognition (ASR) systems have been shown to be vulnerable to adversarial examples (AEs). Recent success all assumes that users will not notice or disrupt the attack process despite the existence of music/noise-like sounds and spontaneous responses from voice assistants. Nonetheless, in practical user-present scenarios, user awareness may nullify existing attack attempts that launch unexpected sounds or ASR usage. In this paper, we seek to bridge the gap in existing research and extend the attack to user-present scenarios. We propose VRIFLE, an inaudible adversarial perturbation (IAP) attack via ultrasound delivery that can manipulate ASRs as a user speaks. The inherent differences between audible sounds and ultrasounds make IAP delivery face unprecedented challenges such as distortion, noise, and instability. In this regard, we design a novel ultrasonic transformation model to enhance the crafted perturbation to be physically effective and even survive long-distance delivery. We further enable VRIFLE's robustness by adopting a series of augmentation on user and real-world variations during the generation process. In this way, VRIFLE features an effective real-time manipulation of the ASR output from different distances and under any speech of users, with an alter-and-mute strategy that suppresses the impact of user disruption. Our extensive experiments in both digital and physical worlds verify VRIFLE's effectiveness under various configurations, robustness against six kinds of defenses, and universality in a targeted manner. We also show that VRIFLE can be delivered with a portable attack device and even everyday-life loudspeakers.

==> sections/additional.tex <==
%  !TEX root = ../dolphin2.tex




\subsection{Wakeup Authentication Penetration}
The proposed technical approaches can achieve targeted voice command alteration for human-interactive scenarios, however, as for human-absent case, the voice assistant should be woken up first to drive it execute malicious commands. Different from the adversarial examples against ASV~\cite{chen2021fakebob,deng2022fencesitter} which only optimizes the expectation problem of bypassing the ASV, an adversary should satisfy both voiceprint matching and speech recognized as the correct wakeup phrase $Y_w$, such as ``Hey Siri''.
Since the attacker accesses to only 1\textasciitilde3 victim's utterance samples unrelated to the wakeup phrase, we apply the text-to-speech (TTS) tool for synthesizing ``Hey Siri'', meeting the wakeup word recognition requirement firstly. As overlaying adversarial noise to manipulate the voiceprint will also affect the speech recognition,
we consider a joint optimization of speaker embedding similarity (voiceprint loss $\mathcal{L}_{ASV}$) and speech recognition accuracy (CTC loss $\mathcal{L}_{CTC}$) based on above methods. Namely, we aim to find a perturbation $\delta_w$ making the overall voiceprint after superimposing synthesized audio $x_{tts}$ close to the original victim's, it still ensures the wakeup word recognized correctly.
Moreover, we especially splice the perturbation with the beginning or end of the original audio, compared to overlaying it on the audio's middle region, the semantic information is well preserved, and the $\mathcal{L}_{CTC}$ can converge faster from the speech recognition perspective, which greatly reduces the complexity of our optimization as follows:

\begin{equation}
    \delta_{w} = \underset{\delta_w}{\operatorname{argmin}}[\mathcal{L}_{ASV}(x_{tts}+\delta_w, x_{vic}) + \alpha\mathcal{L}_{CTC}(x_{tts}+\delta_w,Y_w)]
\end{equation}
where $L_{ASV}$ is the inverse cosine similarity score between the speaker embedding of $x_{tts}+\delta_w$ and $x_{vic}$ that are extracted by the state-of-the-art speaker verfication model ECAPA-TDNN~\cite{2020ecapatdnn}. We empirically set $\alpha$ to 0.01, which is a hyper-parameter adjusting the weights of two losses.

==> sections/proof_of_concept.tex <==
%  !TEX root = ../dolphin2.tex

\section{Attack on Speaker Identification}
Given \alias's remarkably universal capacity to manipulate the ASR, we are motivated to investigate whether such an attack can generalize to speaker identification (SI) systems. We perform an experiment to validate the feasibility. Specifically, we maintain the same design as above while we reconfigure the optimization goal $y_t$ as the target speaker label and the loss function $\mathcal{L}(f(\cdot),y_t)$ as the cosine similarity scoring module.\\
\textbf{Setup:} We employ the state-of-the-art ECAPA-TDNN~\cite{2020ecapatdnn} as our target model and randomly select 10 speakers for evaluation from the popular LibriSpeech dataset~\cite{panayotov2015librispeech} (test-clean). We choose one utterance for creating perturbation and 100 samples for testing from each speaker. The duration of \alias is set to $1s$. We adopt success rate to indicate the percentage of \alias successfully deceiving the SI model and matching the target speaker in all attempts.\\
\textbf{Experiment:} The adversaries aim to tailor an inaudible UAP that can tamper with other speakers' utterances, and the superimposed audio is further extracted into a voiceprint highly similar to the target speaker's. We assume that adversaries can only obtain an utterance from each speaker in this set, and each speaker is treated as a target for UAP crafting, respectively, i.e., 10 perturbations will be created. We apply the UAPs on all test samples of 9 speakers with 10 varying delays, and collect 9,000 samples in each targeted attack attempt. In Fig.~\ref{fig:eval_SI}, each cell shows the average attack success rate, and only 6 out of 90 combinations have average attack success rates under 90\%, with the lowest attack success rate being 83.\%. The overall average attack success rate is 96.9\%, suggesting our generated UAP has good generality over unseen speech.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.28\textwidth]{eval_SI.pdf}
    \caption{\label{fig:eval_SI}Attack performance on speaker identification.}
    % \vspace{-10pt}
\end{figure}

